Clustering high dimensional meteorological scenarios: results and performance index

The Reseau de Transport d'Electricit\'e (RTE) is the French main electricity network operational manager and dedicates large number of resources and efforts towards understanding climate time series data. We discuss here the problem and the methodology of grouping and selecting representatives of possible climate scenarios among a large number of climate simulations provided by RTE. The data used is composed of temperature times series for 200 different possible scenarios on a grid of geographical locations in France. These should be clustered in order to detect common patterns regarding temperatures curves and help to choose representative scenarios for network simulations, which in turn can be used for energy optimisation. We first show that the choice of the distance used for the clustering has a strong impact on the meaning of the results: depending on the type of distance used, either spatial or temporal patterns prevail. Then we discuss the difficulty of fine-tuning the distance choice (combined with a dimension reduction procedure) and we propose a methodology based on a carefully designed index.

==> secs/UCR.tex <==
\subsubsection{Efficiency of the index on diverse (labeled) time series data set}

MLCC distance is likely to be the most interesting method for many cases where
similar patterns should be found in the time series at an intermediate (not too small) time scale. 
We show here that our index works well on many data sets of labelled time series at least when MLCC is the best method among many others.


The UCR series datasets is a set of labeled temporal series datasets.
In order to evaluate our metric we will compare the distance chosen by our index with the one selected using the accuracy. \textcolor{red}{add definition of accuracy}

Since the labels name does not matter, we need to rename the labels obtained by the clustering algorithm to match the true labels. To choose which label is assigned to which label, we will use the assignment that maximizes the accuracy.

From UCR data set, we considered 103 datasets (datasets of variable length were excluded) and the same 7 distances used for RTE dataset.



\begin{table}[H]
\centering
\begin{tabular}{|l|l|l|}
\hline
\multicolumn{2}{|l|}{\textbf{Index for selecting a metric}}                                               & \textbf{\begin{tabular}[c]{@{}l@{}}Proportion of datasets in \\ which the selected metric \\ maximizes the accuracy\end{tabular}} \\ \hline
$F(d) \times Q(d)$ & \begin{tabular}[c]{@{}l@{}}L2 as reference \\ for the fidelity index\end{tabular} &    0.029412                                                                                                                                          \\ \hline
$F(d) \times Q(d)$ & \begin{tabular}[c]{@{}l@{}}DTW as reference \\ for the fidelity index\end{tabular}       &     0.264706                                                                                                                                          \\ \hline
$F(d) \times Q(d)$ & \begin{tabular}[c]{@{}l@{}}MLCC as reference \\ for the fidelity index\end{tabular}   &          0.245098                                                                                                                                    \\ \hline
\multicolumn{2}{|l|}{Always Euclidean}                                                                    &       0.029412                                                                                                                                        \\ \hline
\multicolumn{2}{|l|}{Always DTW}                                                                          &        0.254902                                                                                                                                        \\ \hline
\multicolumn{2}{|l|}{Always MLCC}                                                                      &     0.245098                                                                                                                                         \\ \hline
\multicolumn{2}{|l|}{Expected by random}                                                                  & 1/7 = 0.1428                                                                                                                                       \\ \hline
\end{tabular}
\caption{results for UCR datasets}
\end{table}



\begin{table}[H]
\begin{tabular}{|l|l|l|l|}
\hline
\textbf{Metric with best accuracy}   & \textbf{\begin{tabular}[c]{@{}l@{}}Number of \\ data sets\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}Reference metric \\ for our index\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}prop. of datasets \\ where it selects \\ the metric\\ with best acc.\end{tabular}} \\ \hline
MLCC                               & 99                                                                         & MLCC                                                                                & 33/99 = 0.33                                                                                                                              \\ \hline
MLCC                               & 99                                                                         & dtw                                                                                   & 1/99 = 0.01                                                                                                                              \\ \hline
MLCC                               & 99                                                                         & l2                                                                                    & 1/99 = 0.01                                                                                                                              \\ \hline
dtw                                  & 99                                                                         & MLCC                                                                                & 0/99 = 0.00                                                                                                                               \\ \hline
dtw                                  & 99                                                                         & dtw                                                                                   & 33/99 = 0.33                                                                                                                              \\ \hline
dtw                                  & 99                                                                         & l2                                                                                    &0/99 = 0.00                                                                                                                              \\ \hline
other (haar95, fourier95, PCA95, L2) & 108                                                                         & MLCC                                                                                & 0/108 = 0.00                                                                                                                               \\ \hline
other (haar95, fourier95, PCA95, L2) & 108                                                                         & dtw                                                                                   & 0/108 = 0.00                                                                                                                              \\ \hline
other (haar95, fourier95, PCA95, L2) & 108                                                                         & l2                                                                                    & 11/108 = 0.10                                                                                                                              \\ \hline
\end{tabular}
\caption{Results on UCR dataset}
\end{table}

